Implicit Polarized F: local type inference for impredicativity

System F, the polymorphic lambda calculus, features the principle of impredicativity: polymorphic types may be (explicitly) instantiated at other types, enabling many powerful idioms such as Church encoding and data abstraction. Unfortunately, type applications need to be implicit for a language to be human-usable, and the problem of inferring all type applications in System F is undecidable. As a result, language designers have historically avoided impredicative type inference. We reformulate System F in terms of call-by-push-value, and study type inference for it. Surprisingly, this new perspective yields a novel type inference algorithm which is extremely simple to implement (not even requiring unification), infers many types, and has a simple declarative specification. Furthermore, our approach offers type theoretic explanations of how many of the heuristics used in existing algorithms for impredicative polymorphism arise.

==> proofs-typing-soundness-application-of-weakly-extended-context-subsumes.tex <==
\begin{center}
  \WeakContextAppSubsumption*
\end{center}

\begin{proof}
  By rule induction over the definition of weak context extension.

  \begin{itemize}
    \DerivationProofCase{\Wcempty}
    {}
    {\congoesWeakJudg{\cdot}{\cdot}}

    \begin{llproof}
      \eqPf{[\cdot]([\cdot]A)}{[\cdot]A}{By definition}
    \end{llproof}

    \DerivationProofCase{\Wcuvar}
    {\congoesWeakJudg{\Theta}{\Theta'}}
    {\congoesWeakJudg{\Theta, \alpha}{\Theta', \alpha}}

    \begin{llproof}
      \conwfPf{\Theta, \alpha}{Assumption}
      \conwfPf{\Theta}{Inversion (\cwfuvar)}
      \conwfPf{\Theta', \alpha}{Assumption}
      \conwfPf{\Theta'}{Inversion (\cwfuvar)}
      \proofsep
      \eqPf{[\Theta', \alpha]([\Theta, \alpha]A)}{[\Theta', \alpha]([\Theta]A)}{By definition}
      \continueeqPf{[\Theta']([\Theta]A)}{By definition}
      \continueeqPf{[\Theta']A}{\byih}
      \continueeqPf{[\Theta', \alpha]A}{By definition}
    \end{llproof}

    \DerivationProofCase{\Wcunsolvedguess}
    {\congoesWeakJudg{\Theta}{\Theta'}}
    {\congoesWeakJudg{\Theta, \guess{\alpha}}{\Theta', \guess{\alpha}}}

    \begin{llproof}
      \conwfPf{\Theta, \guess{\alpha}}{Assumption}
      \conwfPf{\Theta}{Inversion (\cwfunsolvedguess)}
      \conwfPf{\Theta', \guess{\alpha}}{Assumption}
      \conwfPf{\Theta'}{Inversion (\cwfunsolvedguess)}
      \proofsep
      \eqPf{[\Theta', \guess{\alpha}]([\Theta, \guess{\alpha}]A)}{[\Theta', \guess{\alpha}]([\Theta]A)}{By definition}
      \continueeqPf{[\Theta']([\Theta]A)}{By definition}
      \continueeqPf{[\Theta']A}{\byih}
      \continueeqPf{[\Theta', \guess{\alpha}]A}{By definition}
    \end{llproof}

    \DerivationProofCase{\Wcsolvedguess}
    {\congoesWeakJudg{\Theta}{\Theta'}}
    {\congoesWeakJudg{\Theta, \guess{\alpha} = P}{\Theta', \guess{\alpha} = P}}

    \begin{llproof}
      \conwfPf{\Theta, \guess{\alpha} = P}{Assumption}
      \conwfPf{\Theta}{Inversion (\cwfsolvedguess)}
      \conwfPf{\Theta', \guess{\alpha} = P}{Assumption}
      \conwfPf{\Theta'}{Inversion (\cwfsolvedguess)}
      \proofsep
      \eqPf{[\Theta', \guess{\alpha} = P]([\Theta, \guess{\alpha} = P]A)}{[\Theta', \guess{\alpha} = P]([\Theta][P / \guess{\alpha}]A)}{By definition}
      \continueeqPf{[\Theta']([P / \guess{\alpha}]([\Theta][P / \guess{\alpha}]A))}{By definition}
      \continueeqPf{[\Theta'][\Theta]([P / \guess{\alpha}][P / \guess{\alpha}]A)}{$[\Theta]-$ substitutes grounds}
      \continueeqPf{[\Theta'][\Theta]([P / \guess{\alpha}]A)}{$\groundJudge{P}$}
      \continueeqPf{[\Theta']([P / \guess{\alpha}]A)}{\byih}
      \continueeqPf{[\Theta', \guess{\alpha} = P]A}{By definition}
    \end{llproof}

    \DerivationProofCase{\Wcsolveguess}
    {\congoesWeakJudg{\Theta}{\Theta'}}
    {\congoesWeakJudg{\Theta, \guess{\alpha}}{\Theta', \guess{\alpha} = P}}

    \begin{llproof}
      \conwfPf{\Theta, \guess{\alpha}}{Assumption}
      \conwfPf{\Theta}{Inversion (\cwfunsolvedguess)}
      \conwfPf{\Theta', \guess{\alpha} = P}{Assumption}
      \conwfPf{\Theta'}{Inversion (\cwfsolvedguess)}
      \proofsep
      \eqPf{[\Theta', \guess{\alpha} = P]([\Theta, \guess{\alpha}]A)}{[\Theta', \guess{\alpha} = P]([\Theta]A)}{By definition}
      \continueeqPf{[\Theta'][P / \guess{\alpha}]([\Theta]A)}{By definition}
      \continueeqPf{[\Theta'][\Theta]([P / \guess{\alpha}]A)}{$[\Theta]-$ substitutes grounds}
      \continueeqPf{[\Theta']([P / \guess{\alpha}]A)}{\byih}
      \continueeqPf{[\Theta', \guess{\alpha} = P]A}{By definition}
    \end{llproof}

    \DerivationProofCase{\Wcunsolvedextend}
    {\congoesWeakJudg{\Theta}{\Theta'}}
    {\congoesWeakJudg{\Theta}{\Theta', \guess{\alpha}}}

    \begin{llproof}
      \conwfPf{\Theta}{Assumption}
      \conwfPf{\Theta', \guess{\alpha}}{Assumption}
      \conwfPf{\Theta'}{Inversion (\cwfunsolvedguess)}
      \proofsep
      \eqPf{[\Theta', \guess{\alpha}]([\Theta]A)}{[\Theta']([\Theta]A)}{By definition}
      \continueeqPf{[\Theta']A}{\byih}
      \continueeqPf{[\Theta', \guess{\alpha}]A}{By definition}
    \end{llproof}

    \DerivationProofCase{\Wcsolvedextend}
    {\congoesWeakJudg{\Theta}{\Theta'}}
    {\congoesWeakJudg{\Theta}{\Theta', \guess{\alpha}} = P}

    \begin{llproof}
      \conwfPf{\Theta}{Assumption}
      \conwfPf{\Theta', \guess{\alpha} = P}{Assumption}
      \conwfPf{\Theta'}{Inversion (\cwfsolvedguess)}
      \proofsep
      \eqPf{[\Theta', \guess{\alpha} = P]([\Theta]A)}{[\Theta'][P / \guess{\alpha}]([\Theta]A)}{By definition}
      \continueeqPf{[\Theta'][\Theta]([P / \guess{\alpha}]A)}{Since $[\Theta]-$ only substitutes non-ground types}
      \continueeqPf{[\Theta']([P / \guess{\alpha}]A)}{\byih}
      \continueeqPf{[\Theta', \guess{\alpha} = P]A}{By definition}
    \end{llproof}
  \end{itemize}
\end{proof}


==> shared-definitions-well-formed-type.tex <==
\judgbox{\wfposnegtypeJudg{\acontext}{A}}{In the context $\acontext$, $A$ is a well-formed positive/negative type}

\begin{mathpar}
  \Infer{\twfuvar}
    {\alpha \in \ConUV(\acontext)}
    {\wfpostypeJudg{\acontext} {\alpha}}
  
  \Infer{\twfguess}
    {\guess{\alpha} \in \EV(\acontext)}
    {\wfpostypeJudg{\acontext} {\guess{\alpha}}}

  \Infer{\twfshiftdown}
    {\wfnegtypeJudg{\acontext} {N}}
    {\wfpostypeJudg{\acontext} {\shiftdown N}}

  \Infer{\twfforall}
    {\wfnegtypeJudg{\acontext, \alpha} {N}}
    {\wfnegtypeJudg{\acontext} {\forall \alpha \ldotp N}}

  \Infer{\twfarrow}
    {\wfpostypeJudg{\acontext} {P} \\ \wfnegtypeJudg{\acontext} {N}}
    {\wfnegtypeJudg{\acontext} {P \funarrow N}}

  \Infer{\twfshiftup}
    {\wfpostypeJudg{\acontext} {P}}
    {\wfnegtypeJudg{\acontext} {\shiftup P}}
\end{mathpar}

